$\P$ILCRO: Making Importance Landscapes Flat Again

Convolutional neural networks have had a great success in numerous tasks, including image classification, object detection, sequence modelling, and many more. It is generally assumed that such neural networks are translation invariant, meaning that they can detect a given feature independent of its location in the input image. While this is true for simple cases, where networks are composed of a restricted number of layer classes and where images are fairly simple, complex images with common state-of-the-art networks do not usually enjoy this property as one might hope. This paper shows that most of the existing convolutional architectures define, at initialisation, a specific feature importance landscape that conditions their capacity to attend to different locations of the images later during training or even at test time. We demonstrate how this phenomenon occurs under specific conditions and how it can be adjusted under some assumptions. We derive the P-objective, or PILCRO for Pixel-wise Importance Landscape Curvature Regularised Objective, a simple regularisation technique that favours weight configurations that produce smooth, low-curvature importance landscapes that are conditioned on the data and not on the chosen architecture. Through extensive experiments, we further show that P-regularised versions of popular computer vision networks have a flat importance landscape, train faster, result in a better accuracy and are more robust to noise at test time, when compared to their original counterparts in common computer-vision classification settings.

==> batchnorm.tex <==
% \subsection{Batch normalisation}
The expected squared partial derivative of the output of a convolutional layer is equal to:
\begin{equation}
    \mathbb{E}_{\bm{j}, \tens{W}, \tens{H}}\left[\left(\frac{\partial a^{(l+1)}_{\bm{j}}}{\partial h^{(l)}_{\bm{i}}}\right)^2\right] = \frac{1}{Z} \mathbb{V}\left[w^{(l)}\right] \mathbb{E}_{\bm{j}}\left[\# p_{a^{(l+1)}_{\bm{j}} \rightarrow h^{(l)}_{\bm{i}}}\right], \, C_{\text{in}} \leq \mathbb{E}_{\bm{j}}\left[\# p_{a^{(l+1)}_{\bm{j}} \rightarrow h^{(l)}_{\bm{i}}}\right] \leq C_{\text{in}}  \prod_{k} \kappa_i
\end{equation}

The partial derivative of $BatchNorm$ layers takes two generic forms, 
\[
\frac{\partial BatchNorm(a^{(l)}_{\bm{j}}, \tens{A}^{(l)})}{\partial a^{(l)}_{\bm{i}}} = \left\{\begin{array}{ll}
     \gamma \frac{N^{(l)}-1}{N^{(l)} \sigma(\bm{A}_{c_{\text{out}}}^{(l)})} - \frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma\left(\bm{A}_{c_{\text{out}}}^{(l)}\right)^3}& \text{ if } j = i \\
     \gamma \frac{-1}{N^{(l)} \sigma\left(\bm{A}_{c_{\text{out}}}^{(l)}\right)}  - \frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma\left(\bm{A}_{c_{\text{out}}}^{(l)}\right)^3}& \text{ otherwise}
\end{array}\right.
\]
from which we can derive the squared derivative:
\begin{equation}\label{eq:sq_deriv_bn}
    \begin{aligned}
\left(\frac{\partial BatchNorm(a^{(l)}_{\bm{j}}, \tens{A}^{(l)})}{\partial a^{(l)}_{\bm{i}}}\right)^2 &= 
\left\{\begin{array}{ll}
     \gamma^2 \left(\frac{N^{(l)}-1}{N^{(l)}}\right)^2 \frac{1}{\sigma\left(\bm{A}^{(l)}_{c_{\text{out}}}\right)^2} + \left(\frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma(\bm{A}^{(l)}_{c_{\text{out}}})^3}\right)^2 - 2 \frac{N-1}{N^{(l)} \sigma(\bm{A}^{(l)}_{c_{\text{out}}})} \frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma(\bm{A}^{(l)}_{c_{\text{out}}})^3} & \text{ if } j = i \\
     \gamma^2 \left(\frac{-1}{N^{(l)}}\right)^2 \frac{1}{\sigma\left(\bm{A}^{(l)}_{c_{\text{out}}}\right)^2} + \left(\frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma(\bm{A}^{(l)}_{c_{\text{out}}})^3}\right)^2 - 2 \frac{-1}{N^{(l)} \sigma(\bm{A}^{(l)}_{c_{\text{out}}})} \frac{\left(a_{\bm{i}} - \overline{\bm{A}_{c_{\text{out}}}^{(l)}}\right)^2}{N \sigma(\bm{A}^{(l)}_{c_{\text{out}}})^3} & \text{ otherwise}
\end{array}\right.\\
&=\left\{\begin{array}{ll}
     \gamma^2 \left(\frac{N^{(l)}-1}{N^{(l)}}\right)^2 \frac{1}{\sigma\left(\bm{A}^{(l)}_{c_{\text{out}}}\right)^2} + \mathcal{O}\left(N^{(l)}\right)^{-2} & \text{ if } j = i \\
     \mathcal{O}\left(\left(N^{(l)}\right)^{-2}\right) & \text{ otherwise.}
\end{array}\right.
\end{aligned}
\end{equation}
Equation~\ref{eq:sq_deriv_bn} shows that we can derive upper bound the squared derivative of the $BatchNorm$ layer, which is tight when the sample size (typically equal to the product of the batch size, the width and the height of the layer considered) is high.

Let us now derive the expected value of the squared partial derivative of the $BatchNorm \circ Conv$ composite function:
\begin{align*}
    &\mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[\left( \frac{\partial \left. BatchNorm\left(a_{\bm{j}}^{(l)}, \tens{A}^{(l)}\right) \right|_{\tens{A} = \tens{W}^{(l-1)} * \tens{H}^{(l-1)}} }{\partial h^{(l-1)}_{\bm{i}}} \right)^2\right] \approx\\
    &\quad\mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[ \gamma^2 \left(\frac{N^{(l)}-1}{N^{(l)}}\right)^2 \frac{1}{\sigma\left(\bm{A}^{(l)}_{c_{\text{out}}}\right)^2} \left(\frac{\partial a_{\bm{j}}}{h_{\bm{i}^{(l-1)}}}\right)^2  \right]
\end{align*}
where the expectation is taken \textit{w.r.t.} the weight distribution and the input data.
We lower bound this expression using Jensen's inequality for the inverse variance expectation
\begin{equation*}
    \begin{aligned}
        \mathbb{E}\left[\frac{1}{\sigma(x)^2}\right] &\geq \frac{1}{\mathbb{E}\left[\sigma(x)^2\right]}\\
        &=\frac{N}{N-1} \frac{1}{\mathbb{V}[x]},
    \end{aligned}
\end{equation*} 
which has an error of the order $\mathcal{O}\left({\left(N^{(l)}\right)^{-1}}\right)$, again making this approximation tight for large $N^{(l)}$:
\begin{equation}\label{eq:exp_sq_composite}
\begin{aligned}
    \mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[\left( \frac{\partial \left. BatchNorm\left(a_{\bm{j}}^{(l)}, \tens{A}^{(l)}\right) \right|_{\tens{A} = \tens{W}^{(l-1)} * \tens{H}^{(l-1)}} }{\partial h^{(l-1)}_{\bm{i}}} \right)^2\right] \approx
    \\\quad \mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[ \gamma^2 \frac{N^{(l)}-1}{N^{(l)}} \frac{1}{\mathbb{V}\left[\bm{A}^{(l)}_{c_{\text{out}}}\right]} \left(\frac{\partial a_{\bm{j}}}{h_{\bm{i}^{(l-1)}}}\right)^2\right].
\end{aligned}
\end{equation}

Using the rule of the total expectation, and noting that under the assumption that the entries of $\tens{H}^{(l-1)}$ are \textit{iid.}, the variance of the output of the convolution is equal to 
\[
\mathbb{V}_{\tens{H}^{(l-1)}}\left[\bm{A}^{(l)}_{c_{\text{out}}}\right] = \mathbb{V}\left[h^{(l-1)}\right] \sum_k \sum_{c_{\text{in}}}
\left(w^{(l-1)}_{k,c_{\text{out}},c_{\text{in}}}\right)^{2}
\]
% \mathbb{E}_{\bm{i},\bm{j}} \left[\# p_{a_{\bm{j}}^{(l)} \rightarrow h_{\bm{i}}^{(l)}}\right]
Equation~\ref{eq:exp_sq_composite} can be decomposed as
\begin{equation}\label{eq:bn_effect}
\begin{aligned}
    &\mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[\left( \frac{\partial \left. BatchNorm\left(a_{\bm{j}}^{(l)}, \tens{A}^{(l)}\right) \right|_{\tens{A} = \tens{W}^{(l-1)} * \tens{H}^{(l-1)}} }{\partial h^{(l-1)}_{\bm{i}}} \right)^2\right]
\\&\quad \approx \mathbb{E}_{\bm{j},\tens{W}^{(l-1)},\gamma}\left[  \gamma^2 \frac{N^{(l)}-1}{N^{(l)}} \frac{1}{ \mathbb{V}\left[h^{(l-1)}\right] \sum_k \sum_{c_{\text{in}}}
\left(w^{(l-1)}_{k,c_{\text{out}},c_{\text{in}}}\right)^{2} } \left(\frac{\partial a_{\bm{j}}}{h_{\bm{i}^{(l-1)}}}\right)^2  \right]\\
&\quad = \mathbb{E}_{\bm{j},\tens{W}^{(l-1)},\gamma}\left[  \gamma^2 \frac{N^{(l)}-1}{N^{(l)}} \frac{1}{ \mathbb{V}\left[h^{(l-1)}\right] \sum_k \sum_{c_{\text{in}}}
\left(w^{(l-1)}_{k,c_{\text{out}},c_{\text{in}}}\right)^{2} } \left(w^{(l-1)}_{\bm{k}}\right)^2  \right]\\
&\quad=\mathbb{E}_{\bm{j},\tens{H}^{(l-1)},\tens{W}^{(l-1)},\gamma}\left[ \gamma^2 \frac{N^{(l)}-1}{N^{(l)}} \frac{1}{ \mathbb{V}\left[h^{(l-1)}\right] \argmax_{\bm{i}}\mathbb{E}_{\bm{j}'}\left[\# p_{a^{(l)}_{\bm{j}'}\rightarrow h^{(l-1)}_{\bm{i}}}\right] } \# p_{a^{(l)}_{\bm{j}}\rightarrow h^{(l-1)}_{\bm{i}}}  \right]\\
&\quad=\frac{N^{(l)}-1}{N^{(l)}}\mathbb{E}_{\gamma}\left[\gamma^2\right] \mathbb{E}_{\bm{j}}\left[\frac{\# p_{a^{(l)}_{\bm{j}}\rightarrow h^{(l-1)}_{\bm{i}}}}{\argmax_{\bm{i}}\mathbb{E}_{\bm{j}'}\left[\# p_{a^{(l)}_{\bm{j}'}\rightarrow h^{(l-1)}_{\bm{i}}}\right]}\right]\frac{1}{ \mathbb{V}\left[h^{(l-1)}\right]} 
\end{aligned}
\end{equation}
where $\bm{k}$ is the index of the weight entry \textit{s.t.} $a_{\bm{j}} = w^{(l-1)}_{\bm{k}} h^{(l-1)}_{\bm{i}}$.
It becomes apparent in Equation~\ref{eq:bn_effect} that $BatchNorm$ layers cancel the effect of the variance of convolutional layers, ensuring that the expected squared partial derivative of the output layer is in good approximation dependent of the input variance only.

The generalization to multiple layers follows by simple recursivity.

==> nonlinearities.tex <==
\section{Effect of nonlinearities}\label{sec:app:NonLinearities}
Nonlinear activation functions and other operations (typically normalization at train time) break the above logic and make the expected squared output-input partial derivative dependent on other factors than the number of paths and the weights variance.
This means that the expected feature importance is not independent of the data anymore, and the picture is therefore more complex.

Here, we focus on the Restricted Linear Unit (ReLU) activation function (\cite{Nair2010}).
Consider the squared partial derivative of the operation $h^{(l)} = ReLU\left(a^{(l)}\right)$:
\begin{align}
\left(\frac{\partial h^{(l)}}{\partial a^{(l)}}\right)^2 = \left \{ \begin{array}{ll} 
1 & \text{if } a^{(l)} > 0\\
0 & \text{otherwise}
\end{array}
\right.
\end{align}
which is on expectation equal to $\frac{1}{2}$ if $a^{(l)}$ is equal to $0$ on expectation.
For later, it will be interesting to remember that, assuming that $\tens{A}^{(l)}$ entries are \textit{i.i.d.} and follow a normal distribution $\mathbb{N}(0, S)$, the output variance is equal to
\begin{equation*}
    \mathbb{V}\left[h^{(l)}\right] = \frac{\mathbb{V}_{x \sim \mathbb{N}^+}[x]}{2} - \left(\frac{\mathbb{E}_{x \sim \mathbb{N}^+}[x]}{2}\right)^2
\end{equation*}
where $\mathbb{N}^+$ is a $[0, \infty)$ truncated normal distribution. 

% After the cell values of the layer $l-1$ have been passed through the convolutional layer $conv^{(l)}$, the partial derivative of the average post-activation $\overline{h}^{(l)} = \frac{1}{N^{(l)}}\sum_{j=1}^{N^{(l)}}\text{ReLU}(a^{(l)}_j)$ where $\bm{a}^{(l)} = conv^{(l)}(\bm{h}^{(l-1)}))$ wrt $h^{(l-1)}_{i}$ reads:
% \begin{align}
%     \frac{\partial \overline{h}^{(l)}}{\partial h^{(l-1)}_{i-1}} &=\left \{ \begin{array}{ll}
%         \frac{\partial a^{(l)}_0}{\partial h^{(l-1)}_{i-1}} & \text{ if } a^{(l)}_0 > 0, a^{(l)}_{1,\dots,N^{(l)}}\leq 0\\
%         \frac{\partial a^{(l)}_0+a^{(l)}_1}{\partial h^{(l-1)}_{i-1}} & \text{ if } a^{(l)}_0 > 0, a^{(l)}_1 > 0, a^{(l)}_{2,\dots,N^{(l)}}\leq 0\\
%         \dots
%     \end{array}\right.
% \end{align}
% which gives rise to the following expected squared partial derivative value:
% \begin{align}\label{eq:sq_relu}
%         \mathbb{E}\left[\left(\frac{\partial \overline{h}^{(l)}}{\partial h^{(l-1)}_{i-1}}\right)^2\right]&= \frac{1}{Z} \sum_{\mathbb{U} \subseteq \mathbb{N}^{(l)}}{\mathbb{E}\left[\left(\sum_{u \in \mathbb{U}} \frac{\partial a^{(l)}_u}{\partial h^{(l-1)}_{i-1}}\right)^2\right] \prod_{u \in \mathbb{U}} p(a^{(l)}_u > 0) \prod_{u' \in \left(\mathbb{N}^{(l)} \backslash \mathbb{U}\right)} p(a^{(l)}_{u'} \leq 0)}
% \end{align}
% where the expectation is taken over the distribution of the data and weights. 
% Observe that the partial derivatives $\frac{\partial a^{(l)}_f}{\partial h^{(l-1)}_{i-1}}$ could be simply replaced by the weights that multiply the target cell value given the output cell, which can be equaled to zero if the input cell is not in the receptive field of the output cell.

% Under the restrictive assumption that the elements of $\bm{a}^{(l)}$ are independently distributed and centered around zero (\textit{e.g.} in CNNs lacking biases, such as ResNet), we can see that the product of probabilities on the \textit{rhs.} of Equation~\ref{eq:sq_relu} reduces to a one half to the power of the number of output units that have $h^{(l-1)}_{i-1}$ in their receptive field $r$:
% \begin{align}\label{eq:sq_relu_id}
%         \mathbb{E}\left[\left(\frac{\partial \overline{h}^{(l)}}{\partial h^{(l-1)}_{i-1}}\right)^2\right]&= \frac{1}{Z} \sum_{\mathbb{F} \subseteq \mathbb{N}^{(l)}}{\mathbb{E}\left[\left(\sum_{f \in \mathbb{F}} \frac{\partial a_f}{\partial h^{(l-1)}_{i-1}}\right)^2\right] \left(\frac{1}{2}\right)^{r}}.
% \end{align}
% It then becomes apparent that the unit-to-unit ratios of expected feature importance within a layer are unchanged by the nonlinearity under these specific conditions, and that the salience correction procedure outlined above makes the expected feature importance flat across the input layers.
% Yet, as the elements of the tensor $\bm{a}^{(l)}$ are ordinarily neither independent nor identically distributed, and because the distribution of the data is not known in advance, Equation~\ref{eq:sq_relu} is in general intractable.
% It is therefore hard to know in advance what behaviour will this expected squared gradient have without making strong assumptions about the data distribution.

To some degree, the case of $BatchNorm$ layers is harder to handle.
Training time batch normalization and its derivatives essentially entail a z-scoring of the input value -- most often the output of a convolutional layer -- over some dimension of the input tensor, typically the batch, height and width dimension for two-dimensional CNNs.
The following lemma shows how $BatchNorm$ layers typically impact the \FeatureImportance in a CNN:
\begin{lemma}\label{lemma:bn_importance}
In a neural network where convolutions are interleaved with batch normalization layers, the salience of a given input entry is in good approximation equal to
\begin{equation}\label{eq:definite_bn_importance}
\begin{aligned}
    &\mathbb{E}_{\bm{j},\tens{X},\tens{W},\bm{\gamma}}\left[\left( \frac{\partial y_{\bm{j}} }{\partial x_{\bm{i}}} \right)^2\right] =\\
    &\quad \prod_{l=1}^{(L)}\frac{N^{(l)}-1}{N^{(l)}}\mathbb{E}_{{\gamma^{(l)}}}\left[{\gamma^{(l)}}^2\right] \mathbb{E}_{\bm{j}}\left[\frac{\# p_{a^{(l)}_{\bm{j}}\rightarrow h^{(l-1)}_{\bm{i}}}}{\argmax_{\bm{i}}\mathbb{E}_{\bm{j}'}\left[\# p_{a^{(l)}_{\bm{j}'}\rightarrow h^{(l-1)}_{\bm{i}}}\right]}\right]\frac{1}{ \mathbb{V}\left[h^{(l-1)}\right]} + \mathcal{O}\left(\sum_{l=1}^{(L)} {N^{(l)}}^{-1}\right)
\end{aligned}
\end{equation}
which is independent of the weight variance.
\end{lemma}
\textbf{Proof}:
\input{batchnorm.tex}
\qedwhite

As we can see, $BatchNorm$ layers decouple the variance of the weights of the discrete convolutions from the measure of input unit importance, at the cost of making it a function of the input variance. 



% The derivative of a batch-normalization layer \textit{w.r.t.} its input cell has the following form:
% \begin{align}\label{eq:bnderiv}
%     \frac{\partial BatchNorm(a^{(l)}_i, \bm{a}^{(l)})}{\partial a^{(l)}_i} &= \frac{\partial}{\partial a^{(l)}_i} \gamma \left\{\frac{a^{(l)}_i - \overline{\bm{a}}^{(l)} }{\sigma(\bm{a}^{(l)})} + \gamma\right\}\\
%     &= \gamma \left( \frac{N^{(l)}-1}{N^{(l)} \sigma(\bm{a}^{(l)})} - \frac{\left(a_i^{(l)} - \overline{\bm{a}}^{(l)}\right)^2}{\sum_{j=1}^{N^{(l)}} \left(a_j^{(l)} - \overline{\bm{a}}^{(l)}\right)^2 }  \right)
% \end{align}
% where $\{\gamma,\gamma\}$ are free parameters, and $\sigma$ is the biased estimate estimate of the standard deviation of the batch feature.
% It results from Equation~\ref{eq:bnderiv} that as the batch (or the size of the dimension being averaged over) grows, the partial derivative will tend to 
% \[
% \frac{\partial BatchNorm(a^{(l)}_i, \bm{a}^{(l)})}{\partial a^{(l)}_i} \approx \gamma \frac{N^{(l)}-1}{N^{(l)} \sigma(\bm{a}^{(l)})}, \, N^{(l)} \gg 0
% \]
% which can be considered as constant \textit{w.r.t.} $a^{(l)}_j$ for values of $a^{(l)}_j$ that are close enough to $\overline{\bm{a}}^{(l)}$.
% For small batch sizes, however, the value correction applied by $KingConv$ layers has the an undesirable effect, expressed by the following lemma: 





% ==========

% \begin{lemma}
% In a CNN limited to $KingConv$-type convolutions interleaved with $BatchNorm$ layers, and assuming that both the input values and weights of the network are identically distributed, the expected squared partial derivative of the average output of the network is greater for corrected input units than for non-corrected units.
% \end{lemma}


% \textbf{Proof:}
% Since $a_j^{(l)}$ results from the inner product of two tensors $\bm{c}^{(l)} \odot \bm{h}^{(l-1)}_{j}$ and $\bm{w}^{(l)}$, where the first is not identically distributed anymore due to the normalization, the second part of the gradient formula in Equation~\ref{eq:bnderiv} will behave in such a way that the ratio of the squared distance to the sum of squared distances will be, on average, greater for some cells (typically, the edges and corners) than others, ultimately resulting in a greater squared partial derivative \textit{w.r.t.} the input values that were ignored before correction. In other words, assuming that $\bm{h}^{(l-1)}$ and $\bm{a}^{(l-1)}$ are both \textit{iid.}, if
% \[
% \exists\,\left\{\{a_i^{(l)}, h_j^{(l-1)}\}\,,\{a_{i'}^{(l)}, h_{j'}^{(l-1)}\}\right\}\,\text{s.t.}\, \frac{\partial a_i^{(l)}}{\partial h_j^{(l-1)}} \neq 0, \, c_j^{(l-1)} > 1,\,\frac{\partial a_{i'}^{(l)}}{\partial h_{j'}^{(l-1)}} \neq 0, \, c_{j'}^{(l-1)} = 1
% \]
% then 
% \begin{align}\label{eq:BNinequality}
% \mathbb{E}\left[\left(\frac{\partial BatchNorm(a^{(l)}_i, \bm{a}^{(l)})}{\partial a^{(l)}_i}\right)^2\right] \geq \mathbb{E}\left[\left(\frac{\partial BatchNorm(a^{(l)}_{i'}, \bm{a}^{(l)})}{\partial a^{(l)}_{i'}}\right)^2\right].
% \end{align}
% To generalize this to the whole network, one just needs to observe that the chain rule implies that the expected squared partial derivative of the output \textit{w.r.t.} the input reads:
% \begin{align}\label{eq:ChainRule}
%     &\mathbb{E}\left[\left(\frac{\partial KingConv \circ BatchNorm  \circ \dots KingConv(\bm{x})}{\partial x_{i}}\right)^2\right] \\&\quad= \mathbb{E}\left[\left(\frac{\partial KingConv}{\partial BatchNorm}\frac{\partial BatchNorm}{\partial KingConv}\dots\frac{\partial KingConv(\bm{x})}{\partial x_{i}}\right)^2\right]
% \end{align}
% and that $\mathbb{E}\left[\frac{\partial KingConv}{\partial BatchNorm}\right]$ has a fixed value after initialization, it is easy to see that Equation~\ref{eq:BNinequality} together with Equation~\ref{eq:ChainRule} imply Lemma 1.

% The great difficulty for both $ReLU$ and $BatchNorm$ layers is to keep the summary statistics of the pre-activation values identical, while correcting the salience of the units that are associated with a lower number of paths.
% To do this, we suggest that the gradient of the pre-actication value can be changed during the backward pass in order to account for the mismatch in path number in a way that mimics the effect of changing the input salience. 
% It becomes then apparent that the aforementioned issues disappear: whereas the gradient \textit{w.r.t.} the input values of sequence of operations $\bm{y} = h^{(L)} \circ h^{(l-1)} \circ \dots \circ h^0(\bm{c} \odot \bm{x})$ reads
% \[
% \frac{d \bm{y}}{d \bm{x}} = {h^{(L)}}' {h^{(L-1)}}' \dots {h^0}'(\bm{c}\odot\bm{x}) \odot \bm{c}
% \]
% modifying the gradient only ensured that during backpropagation the number of paths is changed according to the location of the input, whereas the summary statistics of each and every units of the network is unchanged:
% \[
% \frac{d \bm{y}}{d \bm{x}} \triangleq {h^{(L)}}' {h^{(l-1)}}' \dots {h^0}'(\bm{x}) \odot \bm{c}.
% \]

% Take for instance a $KingConv$ layer with weights $\bm{w}^{(l)}$ where the input value has been corrected by an intensity map $\bm{c}^{(l)}_{m \times n}$:
% \[
% \bm{h}^{(l)} = KingConv(\bm{c}^{(l)}_{m \times n} \odot \bm{h}^{(l-1)} ; \bm{w}^{(l)}).
% \]
% The gradient of the average $\overline{\bm{h}}^{(l)}$ \textit{w.r.t.} $\bm{h}^{(l-1)}$ is simply being multiplied by the constant map $\bm{c}^{(l)}_{m \times n}$ with respect to its parent $Conv$ version, whereas the gradient \textit{w.r.t.} $\bm{w}^{(l)}$ can be adapted by a linear combination of the constant weight $\bm{c}^{(l)}_{m \times n}$.

